Paraphrasing, textual entailment, and semantic similarity above word level

This dissertation explores the linguistic and computational aspects of the meaning relations that can hold between two or more complex linguistic expressions (phrases, clauses, sentences, paragraphs). In particular, it focuses on Paraphrasing, Textual Entailment, Contradiction, and Semantic Similarity. In Part I: "Similarity at the Level of Words and Phrases", I study the Distributional Hypothesis (DH) and explore several different methodologies for quantifying semantic similarity at the levels of words and short phrases. In Part II: "Paraphrase Typology and Paraphrase Identification", I focus on the meaning relation of paraphrasing and the empirical task of automated Paraphrase Identification (PI). In Part III: "Paraphrasing, Textual Entailment, and Semantic Similarity", I present a novel direction in the research on textual meaning relations, resulting from joint research carried out on on paraphrasing, textual entailment, contradiction, and semantic similarity.

==> 0_Abstract_Old.tex <==
This dissertation explores the linguistic and computational aspects of the meaning relations that can
hold between two or more complex linguistic expressions (phrases, clauses, sentences, paragraphs).
In particular, I focus on Paraphrasing, Textual Entailment, Contradiction, and Semantic Similarity.
From the linguistic side, I study the nature of the meaning relations and the different linguistic 
phenomena involved in each of them. From the computational side, I analyze and evaluate different
approaches for formalizing and comparing the meaning of words and complex linguistic expressions.
Unlike previous work in the area, I do not limit my research to a single meaning relation. I 
compare the linguistic and computational aspects of the different relations, and I propose a shared
typology for meaning relations as well as a general purpose qualitative evaluation framework, which
can be applied to multiple relations.
This thesis is composed of seven different articles and is broadly divided into three thematical Parts.

%Paraphrasing, Textual Entailment, and Semantic Similarity are relations between the meaning of two
%or more complex linguistic expressions (phrases, clauses, sentences, paragraphs). Determining the
%meaning relation that holds between two expressions in an automatic way is a non-trivial task that 
%requires tools and resources at multiple linguistic levels - morphological, lexical, syntactic, and 
%discourse. The recent popularity of Distributional Semantics and Machine Learning has led to an 
%increased interest in meaning relations and the ways to process them automatically. There has been
%multiple shared tasks, datasets, and practical systems built around Paraphrasing, Textual Entailment,
%and Semantic Similarity. However, despite the time and resources invested, the performance of the 
%systems is still not satisfactory in downstream applications and real-world setup. Furthermore, the
%different relations are mostly studied in isolation, despite the theoretical and practical similarities
%between them. 


%In \textbf{Part \ref{p:dsm}} I study the Distributional Hypothesis, which is central for most contemporary 
%approaches for automatic processing of meaning and meaning relations. I explore some applications of 
%Distributional Semantics on semantic similarity at the levels of words and short phrases. In this section 
%I present two articles. 
%In \textbf{Part \ref{p:type}} I study the nature and definition of the Paraphrasing relation and the 
%practical task of Paraphrase Identification. In this section I present three articles. 
%In \textbf{Part \ref{p:mrel}} I compare different semantic relations (Paraphrasing, Textual Entailment, 
%Contradiction, Textual Specificity, and Semantic Similarity) and explore their interactions. In this section
%I present two articles.

\myparagraph{Part \ref{p:dsm}: Similarity at the Level of Words and Phrases} 
In this Part I study the Distributional Hypothesis, which is central for most contemporary
approaches for automatic processing of meaning and meaning relations. I explore some applications of
Distributional Semantics on semantic similarity at the levels of words and short phrases. This part is 
composed of two articles, presented in Chapters \ref{ch:sepln} and \ref{ch:discover}.
%
%This part focuses on the Distributional Hypothesis (DH) and Distributional 
%Semantics (DS). DH is one of the most influential hypotheses in
%contemporary Computational Linguistics (CL) and Natural Language Processing (NLP) and in particular
%in the sub-fields that focus on representing meaning and recognizing, extracting, or generating meaning
%relations. In this part I study the core concepts of DH and DS and I explore some of their
%practical applications. 

In \underline{Chapter \ref{ch:sepln}} I study the notion of (lexical) distributional similarity and some of the 
ways to formalize and quantify it. I compare different Distributional Similarity Models on the task 
of grouping together semantically related words in English and Spanish languages. 
I also explore the importance of the corpus size and the role of linguistic preprocessing in that task.

In \underline{Chapter \ref{ch:discover}} I study the interaction between (lexical) semantic similarity and
meaning compositionality. I present a methodology that uses groups of semantically related words, syntactic 
dependencies, and machine learning algorithms to automatically generate syntactically and semantically 
coherent short phrases. A large portion of the phrases have not been attested in the corpus. I 
demonstrate that (lexical) semantic similarity can interact with syntactic-based compositional rules and 
result in productive patterns at the phrase level.

%(1) I study the notion of (lexical) semantic similarity in the context of the Distributional Semantics 
%Framework. 
%(2) I explore a methodology that uses semantically similar words to automatically compose semantically 
%and syntactically coherent short phrases. I study the role and function of similar words in the meaning 
%of complex linguistic expressions.
%Both these topics are central in the research on Paraphrasing, Textual Entailment, and Semantic 
%Similarity.
%
%First, I discuss the Distributional Hypothesis, which is central for most of the state-of-the-art
%approaches for determining meaning relations. I explore the notion of (lexical) distributional similarity
%and the ways to formalize and quantify it. I compare different Distributional Similarity
%Models on the task of grouping together semantically related words in English and Spanish languages. 
%I also explore the importance of the corpus size and the role of linguistic preprocessing in the task.

%Second, I present a methodology that uses groups of semantically related words, syntactic 
%dependencies, and machine learning algorithms to automatically generate syntactically and semantically 
%coherent short phrases. A large portion of the phrases have not been attested in the corpus. I 
%demonstrate that lexical similarity can interact with syntactic-based compositional rules and result in 
%productive patterns at the phrase level.

\myparagraph{Part \ref{p:type}: Paraphrase Typology and Paraphrase Identification} 
This Part focuses on the Paraphrasing meaning relation and the task of 
Paraphrase Identification (PI). Paraphrasing is one of the most widely studied meaning relation both 
in theoretical and in practical research. PI is among the popular tasks in contemporary Computational
Linguistics (CL) and Natural Language Processing (NLP) with multiple datasets and many practical systems 
devoted to it. In this Part I argue that the complexity of Paraphrasing is not adequately addressed in the 
existing annotation tools, datasets, tasks, and practical systems. I present a typological approach to 
studying Paraphrasing both in theoretical and in practical setting. The empirical evaluation shows promising 
results and demonstrates clear advantages of my approach compared with the traditional approaches.
This part is composed of three articles, presented in Chapters \ref{ch:warp}, \ref{ch:etpc}, and \ref{ch:peval}.

In \underline{Chapter \ref{ch:warp}} I present WARP-Text, a new multi-functional web-based annotation 
tool. WARP-Text allows for a fine-grained annotation of meaning relations at various linguistic levels. It 
fills an important gap in the existing NLP and CL toolbox. WARP-Text has already been successfully used 
in several annotation tasks.

In \underline{Chapter \ref{ch:etpc}} I present the Extended Typology Paraphrase Corpus (ETPC) - the 
largest corpus to date, annotated with paraphrase types. I also propose the Extended Paraphrase 
Typology (EPT) - a linguistically motivated list of phenomena involved in the paraphrasing relation.

In \underline{Chapter \ref{ch:peval}} I present a Qualitative Evaluation Framework for Paraphrase 
Identification. This is the first empirical approach within PI which is making use paraphrase typology. 
I evaluate 11 different automated Paraphrase Identification systems and empirically demonstrate the 
limitations of the existing resources and systems and the advantages of typological research.

%In the second section of this thesis I study the nature and definition of the Paraphrasing relation and the
%practical task of Paraphrase Identification. I argue that the complexity of Paraphrasing is not 
%adequately addressed in the existing annotation tools, datasets, tasks, and practical systems. I fill these 
%gaps in the Paraphrasing research by (i) creating a new multi-functional annotation tool, (ii) creating 
%a new linguistically conditioned and practically oriented paraphrase typology, (iii) annotating a Paraphrase
%Identification corps with with paraphrase types, and (iv) presenting a novel qualitative evaluation
%framework for paraphrase identification and carrying out an extensive evaluation of existing Paraphrase
%Identification systems. This section presents a new approach to studying Paraphrasing both in theoretical
%and in practical setting. The empirical evaluation shows promising results and demonstrates clear 
%advantages of my approach compared with the traditional approaches.
%
%Paper 1 Summary - annotation tool and usage.
%
%Paper 2 Summary - typology and corpus.
%
%Paper 3 Summary - evaluation.

\myparagraph{Part \ref{p:mrel}: Paraphrasing, Textual Entailment, and Semantic Similarity} 
This Part focuses on the comparison between different meaning relations (Paraphrasing, Textual 
Entailment, Contradiction, Textual Specificity, and Semantic Similarity) and the interactions between
them. This research contrasts the traditional approaches in the field, where each meaning relation is
studied and processed in isolation. I propose a new research direction, which brings all the relations
together in a single framework. This part is composed of two articles, presented in Chapters \ref{ch:law} and \ref{ch:sharel}.

%In the third part of this thesis I compare different semantic relations and explore their interactions. This
%is the first empirical study that brings together relations such as Paraphrasing, Textual Entailment, 
%Contradiction, Textual Specificity, and Semantic Similarity. I compare the relations in two different ways,
%by (i) creating the first corpus that contains all relations of interest with sufficient frequency, and (ii) using
%a typology to annotate and compare pairs of sentences having Paraphrasing, Textual Entailment, Contradiction, 
%and Textual Specificity relations.

In \underline{Chapter \ref{ch:law}} I present a new corpus, containing pairs annotated with Paraphrasing, 
Textual Entailment, Contradiction, Textual Specificity, and Semantic Similarity. I propose a new corpus
creation methodology that can be used to create high quality corpora with multiple relations. I analyze 
the co-occurrence, overlap, and co-dependence of the different relations. I demonstrate the potential of
 a new research direction focused on a general framework for meaning relations.

In \underline{Chapter \ref{ch:sharel}} I present a shared typology for meaning relations. The SHARel
typology is based on EPT, but is extended to cover all meaning relations (Textual Entailment, Contradiction,
Textual Specificity, Semantic Similarity). The typology allows to better understand and compare the various
meaning relations. I analyze the frequencies of the different phenomena across the different relations and
outline the similarities and the differences. The SHARel typology also facilitates the transfer of knowledge 
across the different fields and allows for a qualitative evaluation of multiple tasks.

==> 1_1_Departure.tex <==
%Two points of departure - distributional semantics and meaning relations.
\subsection{Object of Study: Textual Meaning Relations}\label{ch:dep:mr}

The objects of study of this thesis are the meaning relations that can hold between language 
expressions. In particular, I focus on meaning relations between complex language expressions,
such as clauses, sentences, and texts. Processing and understanding meaning relations are 
open problems in the fields of Computational Linguistics (CL) and Natural Language Processing 
(NLP) and are related to a large volume of theoretical work and to several challenging practical 
tasks.

Within the fields of CL and NLP, there is no precise and widely accepted definition for the term 
``meaning relation''. In practice, researchers typically narrow the scope of their work to only a 
few (often just one) particular meaning relation. The most popular textual meaning relations 
include Paraphrasing, Textual Entailment, and Semantic Textual Similarity. The definitions for 
these relations in CL and NLP come from empirical tasks.


The work on meaning relations in CL and NLP goes in two different research directions: 
1) to design and improve systems that are capable of processing meaning relations in an 
automatic manner and 2) to understand the nature and workings of the meaning relations. 
While these two research directions are not mutually exclusive, researchers typically focus 
only on one of them.

\subsection{Empirical Tasks on Meaning Relations}\label{ch:dep:task}

\subsection{Decomposing Meaning Relations}\label{ch:dep:type}

\subsection{Joint Research on Meaning Relation}\label{ch:dep:multi}



The problem of determining the meaning relation, at the most general level, does not have a 
precise and widely accepted definition. In practice, researchers typically narrow the scope of 
their work to only a few (often just one) particular meaning relation. In this thesis I argue
that a joint study of multiple meaning relations will: 1) improve the performance and error 
analysis of the practical tools created for each individual relation; 2) help researchers 
understand the workings of each individual relation; and 3) provide insights on the similarities, 
differences, and interactions between the relations and facilitate the transfer of knowledge
and resources between them.

Typically, there is a distinction between meaning relations at lexical level, henceforth ``lexical
relations'', and meaning relations at the level of complex language expressions, henceforth 
``textual relations''. There is also work on meaning relations at the level of a whole document.
However ``document relations'' fall outside the scope of this thesis.

\myparagraph{Lexical Relations} 


\myparagraph{Human Processing of Meaning Relations}

Human judgments are commonly used in the creation of language resources for the 
research on meaning relations. In recognition tasks, human judgments are the gold 
standard used to evaluate the performance of automated systems.

Despite the high quality of the human judgments, the linguistic and cognitive processes 
underlying these judgments are yet unclear. Some researchers \citep{Sammons,CabrioMagnini} 
argue that determining the presence of a meaning relation is a complex
multi-step inference process. I follow a similar approach in this dissertation and study the 
nature and role of the different ``steps''.

\myparagraph{Automatic Processing of Meaning Relations}

From a theoretical point of view, the automatic processing of meaning relations can 
provide some insights on the workings of the relations. It can also help researchers 
working on more general topics like compositionality of meaning and meaning representation. 
From a more practical side, success in the automatic processing of meaning relations can 
directly affect downstream applications and other empirical tasks in CL and NLP.


\myparagraph{Connections to Other Areas in CL and NLP}


In Table 1 (TO BE ADDED) I have made
a comparison between the different indicating the types that are shared or compatible
across different typologies. I argue that the similarity between the different typologies 
validates the approach that the different authors are taking. For me it also indicates that 
it would be possible to propose a single typology for all meaning relations.




In this thesis I argue that this difference poses a problem both from theoretical and from 
practical point of view. From a theoretical point, understanding the meaning relations
requires understanding and distinguishing the different linguistic and reason-based
phenomena involved in them. From a practical point, the difference in complexity between
instances of meaning relations poses challenges in terms of evaluation and generalizability.



==> 1_5_Terminology.tex <==
In this section I familiarize the reader with some terms relevant to this study and to the
research in the fields of distributional semantics, meaning relations, and machine learning.

\myparagraph{Distributional Semantics}

\myparagraph{Meaning Relations}

In this thesis, we use a very general interpretation of the term \textbf{meaning relations}. 
NEED TO THINK/COPY A DEFINITION OF MEANING RELATIONS.

We distinguish between: 1) \textbf{lexical meaning relations} (also referred to as \textbf{lexical 
relations}): the meaning relations between two words or multi-word expressions; and 2)
\textbf{textual meaning relations} (also referred to as \textbf{textual relations}): the meaning
relations between two complex language expressions (phrases, clauses, and sentences).

This thesis focuses on textual relations. In particular, we study extensively three textual 
relations: paraphrasing, textual entailment, and semantic similarity. We adopt the practical
definitions of these relations, used in the corresponding empirical tasks: Paraphrase Identification.
Recognizing Textual Entailment, and Semantic Textual Similarity.


The practical definition for \textbf{Paraphrasing} is \textit{``whether two 
sentences at the high level ``mean the same thing'' /.../ despite obvious differences in 
information content.''} as formulated by \cite{dolan2005}. Two sentences that are connected
with a paraphrasing relation can be seen in 1.

\begin{itemize}
	\item[(1)] \textbf{Sentence 1:} The genome of the fungal pathogen that causes 
	Sudden Oak Death has been sequenced by US scientists.\\
	\textbf{Sentence 2:} Researchers announced Thursday they've completed the genetic
	blueprint of the blight-causing culprit responsible for sudden oak death.\\
\end{itemize}

The practical definition for \textbf{Textual Entailment} is \textit{``a directional relationship 
between pairs of text expressions, denoted by T - the entailing ``Text'', and H - the entailed 
``Hypothesis''. We say that T entails H if the meaning of H can be inferred from the meaning 
of T, as would typically be interpreted by people.''} as formulated by \cite{rte}. An example 
for textual entailment can be seen in 2. In the given example the Text entails Hyp 1, but not 
Hyp 2, or Hyp 3. 

\begin{itemize}
	\item[(2)] \textbf{Text:} The purchase of Houston-based LexCorp by BMI for \$2Bn
	prompted widespread sell-offs by traders as they sought to minimize exposure. LexCorp 
	had been an employee-owned concern since 2008. \\
	\textbf{Hyp 1:} BMI acquired an American company.\\
	\textbf{Hyp 2:} BMI bought employee-owned LexCorp for \$3.4Bn.\\
	\textbf{Hyp 3:} BMI is an employee-owned concern.\\
\end{itemize}

The practical definition for \textbf{Semantic Similarity} is \textit{``how similar two sentences 
are to each other according to the following scale:\\
\textbf{[5] Completely equivalent}, as they mean the same thing.\\
\textbf{[4] Mostly equivalent}, but some unimportant details differ.\\
\textbf{[3] Roughly equivalent}, but some important information differs/missing.\\
\textbf{[2] Not equivalent}, but share some details. \\
\textbf{[1] Not equivalent}, but are on the same topic \\
\textbf{[0] On different topics.} \\
} as formulated by \cite{sts}. Examples for each semantic similarity from 0 to 5 can be seen in 3.

\begin{itemize}
	\item[(3)] \textbf{Similarity 5:} \\
	The bird is bathing in the sink.  \\
	Birdie is washing itself in the water basin. \\
	\textbf{Similarity 4:} \\
      In May 2010, the troops attempted to invade Kabul. \\
      The US army invaded Kabul on May 7th last year, 2010.\\
	\textbf{Similarity 3:} \\
      John said he is considered a witness but not a suspect.\\
      ``He is not a suspect anymore.'' John said.\\
	\textbf{Similarity 2:} \\
      They flew out of the nest in groups.\\
      They flew into the nest together.\\
	\textbf{Similarity 1:} \\
      The woman is playing the violin.\\
      The young lady enjoys listening to the guitar.\\
	\textbf{Similarity 0:} \\
      John went horse back riding at dawn with a whole group of friends.\\
      Sunrise at dawn is a magnificent view to take in if you wake up
      early enough for it.\\
\end{itemize}

\myparagraph{Practical Tasks and Machine Learning}

==> 1_7_Connect.tex <==
This thesis consists of seven articles, one per chapter, organized in three parts: 

\begin{itemize}
	\item[\ref{p:dsm}] Similarity at the Level of Words and Phrases
	\item[2.] Paraphrase Typology and Paraphrase Identification
	\item[3.] Paraphrasing, Textual entailment, and Semantic Similarity
\end{itemize}

The order of the chapters follows the chronological order in which the articles were written. 
At the same time, the order of the chapters follows the logical progression of my dissertation.
Each of the articles is self sufficient: it poses its own research questions, presents the related 
work and the proposed methodology and then describes the experimental results. However,
there is also a clear thread that connects all the articles. When brought together, the articles
tell a coherent story about the linguistic phenomena involved in textual meaning relations and
how these phenomena can be used to improve the performance of the automated systems 
and bring together multiple textual relations.

In this chapter I briefly present the main motivation, research questions and findings for
each of the three parts and the logical progression of the thesis. I also discuss how each article 
fits within the more general objectives and how the the different articles interact with each
other.

\subsection{Similarity at the Level of Words and Phrases}

The first part of this thesis consists of two articles: 
\begin{itemize}
	\item[1.] Venelin Kovatchev, M. Ant{\`o}nia Mart{\'i}, and Maria Salam{\'o}. 2016. Comparing Distributional Semantics Models for identifying groups of 	semantically related words. \textit{Procesamiento del Lenguaje Natural} vol. 57, pp.: 109-116

	\item[2.] M. Ant{\`o}nia Mart{\'i}, Mariona Taul{\'e}, Venelin Kovatchev,  and Maria Salam{\'o}. 2019. DISCOver: DIStributional approach based on syntactic dependencies for discovering COnstructions. \textit{Corpus Linguistics and Linguistic Theory}
\end{itemize}

This part of the thesis is first chronologically and logically. There were three main objectives
behind this part of my research

My \textbf{first objective for Part I} was to explore the theoretical framework and the empirical tools of the 
Distributional Semantics (DS). DS is the most popular framework in contemporary Natural 
Language Processing (NLP) and Computational Linguistics (CL). The majority of the 
state-of-the-art systems in Paraphrase Identification (PI), Recognizing Textual Entailment 
(RTE), and Semantic Textual Similarity (STS) are based on DS. As such, it was necessary
for me to familiarize with the different theoretical and practical aspects of DS.

My \textbf{second objective for Part I} was to explore the different methodologies for representing the 
meaning of individual words, the different ways to quantitatively compare the meaning
representations, and the different approaches to measuring similarity at the level of
words. This thesis is about textual meaning relations, however the meaning of the 
individual words does contribute to the meaning of the complex language expression. 
This is true in theoretical linguistics and philosophy\footnote{For example, according to Frege's 
principle of semantic compositionality the meaning of a (syntactically complex) whole is 
a function only of the meanings of its (syntactic) parts together with the manner in which 
these parts were combined.} but also in practical applications where machine learning
models often use the vector representations of the individual words to obtain a 
representation of the whole text. Furthermore there are many analogies that can be found 
between lexical relations and textual relations. 

My \textbf{third objective for Part I} was to study the importance of lexical similarity in the
context of complex language expressions. I wanted to study the transition from words to
complex language expressions and to determine to role of semantically related words in
the compositionality of meaning.

With the two articles presented in Part I address all three of the objectives. \textbf{Article 1}, published
in the Journal of the Spanish Society for Computational Linguistics, focuses on objective 1
and 2. In this article I discuss some core concepts and approaches in DS and I present an 
empirical comparison between competing methodologies 
within DS. I explore different methodologies for formalizing the meaning of the words, and
I experiment with different parameters for each model. I apply and compare three 
qualitatively different ways to measure semantic similarity: direct distance in vector space,
clustering, and WordNet similarity. \textbf{Article 2}, published in the ``Corpus Linguistics and Linguistic 
Theory'' journal, addresses all three objectives. In this article, we discuss the different
aspects of DS, we experiment with different ways to formalize and compare the meaning
of words, and finally, we demonstrate how lexical similarity can be used to create unseen
lexico-syntactic patterns.

In Part I of this thesis I successfully experiment with different methodologies and parameters
within DS and I explore one strategy for creating semantically related complex language
expressions - by substituting semantically related words. In the following chapters I identify
other viable strategies within textual meaning relations. I also make use of the knowledge
and resources gathered in this first part.

\subsection{Paraphrase Typology and Paraphrase Identification}

This part of the thesis consists of three articles:
\begin{itemize}
	\item[3.] Venelin Kovatchev, M. Ant{\`o}nia Mart{\'i}, and Maria Salam{\'o}. 2018. WARP-Text: a Web-Based Tool for Annotating Relationships between Pairs of Texts. 	\textit{Proceedings of the 27th International Conference on Computational Linguistics: System Demonstrations}, pp.: 132-136

	\item[4.] Venelin Kovatchev, M. Ant{\`o}nia Mart{\'i}, and Maria Salam{\'o}. 2018. ETPC - a paraphrase identification corpus  annotated with extended paraphrase typology and negation. \textit{Proceedings of the Eleventh International Conference on Language Resources and Evaluation}, pp.: 1384-1392

	\item[5.] Venelin Kovatchev, M. Ant{\`o}nia Mart{\'i}, Maria Salam{\'o}, and Javier Beltran. 2019. A Qualitative Evaluation Framework for Paraphrase Identification. \textit{Proceedings of the Twelfth Recent Advances in Natural Language Processing Conference}, pp.: 569-579
\end{itemize}

There were two main objectives in this part of my research:

My \textbf{first objective for Part II} was to create a large scale corpus for Paraphrase 
Identification, annotated with paraphrase types. While there had been some previous
work on paraphrase typology, at the beginning of my dissertation existed no PI corpus
annotated with paraphrase types. The researchers previously working on paraphrase
or entailment typology provided only a small corpus of examples to illustrate their
proposal. None of these corpora were suitable for an empirical task.

My \textbf{second objective for Part II} was to empirically validate and quantify the 
difference between the paraphrase types. The theoretical work on paraphrase typology
suggests that different paraphrase types require different linguistic and reasoning 
capabilities and the preliminary annotation studies demonstrated that different types 
have different frequency in the PI corpora. However, at the beginning of my dissertation,
paraphrase types were a purely theoretical concept. My objective was to come up with
an experimental setup that can empirically validate whether or not there is a significant 
difference in the way the different paraphrase types are processed by automated PI
systems.

With the three articles presented in Part II, I successfully addressed both objectives.
\textbf{Article 3}, presented as a system demonstration at the 27th International Conference on 
Computational Linguistics in Santa Fe, USA, describes WARP-Text: a new web-based annotation
tool, designed for a fine-grained annotation of multiple texts simultaneously. Without 
such a tool my first objective for annotating a PI corpus with paraphrase types was not
possible. I released the code for WARP-Text to the community and since then it has 
been used in several annotations. \textbf{Article 4}, presented at the Eleventh International 
Conference on Language Resources and Evaluation in Miyazaki, Japan, addresses my
first objective for this Part. In this article I proposed a new paraphrase typology, the
Extended Paraphrase Typology (EPT), which is more expressive than any existing 
paraphrase typology at the time. In this paper I also created and presented ETPC - 
the largest corpus to date annotated with paraphrase types. The size and format of
ETPC make it the first first corpus with paraphrase types that can be used for the task
of PI. \textbf{Article 5}, presented at the Twelfth Recent Advances in Natural Language 
Processing Conference in Varna, Bulgaria, describes a qualitative evaluation framework
for Paraphrase Identification. I propose an experimental setup based on EPT and ETPC,
which can empirically validate the importance and role of the paraphrase types and at
the same time can provide a better evaluation and error analysis of the automated PI 
systems. 

In part II of my thesis I successfully build upon the existing work on decomposing 
paraphrasing and paraphrase typology. I propose a new extended typology, I design
an annotation tool that can facilitate further research and I create the first PI corpus
annotated with paraphrase types. I empirically demonstrate that different paraphrase
types are processed differently by automated PI systems and I suggest a methodology
for automatic qualitative evaluation and error analysis of PI systems. 

\subsection{Paraphrasing, Textual entailment, Semantic Similarity}

This part of the thesis consists of two articles:

\begin{itemize}
	\item[6.] Darina Gold, Venelin Kovatchev, Torsten Zesch. 2019. Annotating and analyzing the interactions between meaning relations \textit{Proceedings of the Thirteenth Language Annotation Workshop}, pp.: 26-36

	\item[7. ] Venelin Kovatchev, Darina Gold, M. Ant{\`o}nia Mart{\'i}, and Maria Salam{\'o}. 2020. A shared typology for paraphrasing, entailment, contradiction, and specificity. Submitted to \textit{Twelfth International Conference on Language Resources and Evaluation}
\end{itemize}

There were two main objectives in this part of my research:

My \textbf{first objective for Part III} was to create a corpus where multiple meaning
relations appear naturally and are explicitly annotated. The existing corpora on meaning
relations was created around only on one or two meaning relations. This setup limits
the possibility to study the relations together and/or to propose more complicated 
empirical tasks involving multiple meaning relations.

My \textbf{second objective for Part III} was to explore the possibility of using a single
typology for all meaning relations. When creating the EPT, I noticed that the typologies
for paraphrasing, textual entailment, and semantic similarity share many of their types.
A single typology for meaning relations would allow for a direct comparison of the 
individual relations and would facilitate the transfer of knowledge between them.

With the two articles presented in Part III I successfully addressed both objectives. 
\textbf{Article 6}, presented at the Thirteenth Language Annotation Workshop, 
co-located with ACL2019 in Florence, Italy, described a methodology for the creation 
and annotation of a corpus of multiple meaning relations. In that article I also analyzed
the correlations and overlap between the different meaning relations and I discussed
the nature of the interactions between them. \textbf{Article 7}, which is currently
under review at the Twelfth International Conference on Language Resources and 
Evaluation, presents SHaRel - a shared typology for multiple meaning relations. In this
paper I discuss the theoretical justification behind the typology, I annotate a corpus 
with the typology and I analyze and compare the frequency of the linguistic phenomena
across four different textual meaning relations.

In part III of my thesis I successfully demonstrate that multiple meaning relations can
appear together in the same corpus. This experiment facilitates future joint work on
meaning relations. I also successfully demonstrate that multiple meaning relations can
be decomposed using the same typology. This discovery facilitates the comparison of
the meaning relations, the transfer of knowledge between them and allows for the
creation of a qualitative evaluation framework that can be applied to multiple meaning
relations.
